Quantum Random Number Generators : Benchmarking and Challenges

We discuss the current state of the art of Quantum Random Number Generators (QRNG) and their possible applications in the search for quantum advantages. To this aim, we first discuss a possible way of benchmarking QRNG by applying them to the computation of complicated and hard to realize classical simulations, such as critical dynamics in two-dimensional Ising lattices. These are performed with the help of computing devices based on field-programmable gate arrays (FPGAs) or graphic processing units (GPUs). The results obtained for QRNG are compared with those obtained by classical pseudo-random number generators (PRNG) of various qualities. Monte Carlo simulations of critical dynamics in moderate lattice sizes (128$\times$128) start to be sensitive to the correlations present in pseudo-random numbers sequences, allowing us to detect them. By comparing our analysis with that of Ref. [PRE {\bf 93}, 022113 (2016)], we estimate the requirements for QRNGs in terms of speed, rapidity of access, and efficiency to achieve the objective of quantum advantage with respect to the best PRNGs. We discuss the technical challenges associated with this objective.

==> test_figures.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \caption{}
        \includegraphics[width=\columnwidth]{images/ratioVarMean.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \caption{}
        \includegraphics[width=\columnwidth]{images/ratioVarMean_reseed.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \caption{}
        \includegraphics[width=\columnwidth]{images/ratioVarMean_reseed_kappalower0.png}
    \end{subfigure}
    \caption{}
\end{figure*}
